User Engagement Prediction for Clarification in Search

Clarification is increasingly becoming a vital factor in various topics of information retrieval, such as conversational search and modern Web search engines. Prompting the user for clarification in a search session can be very beneficial to the system as the user's explicit feedback helps the system improve retrieval massively. However, it comes with a very high risk of frustrating the user in case the system fails in asking decent clarifying questions. Therefore, it is of great importance to determine when and how to ask for clarification. To this aim, in this work, we model search clarification prediction as user engagement problem. We assume that the better a clarification is, the higher user engagement with it would be. We propose a Transformer-based model to tackle the task. The comparison with competitive baselines on large-scale real-life clarification engagement data proves the effectiveness of our model. Also, we analyse the effect of all result page elements on the performance and find that, among others, the ranked list of the search engine leads to considerable improvements. Our extensive analysis of task-specific features guides future research.

==> 7.not_gonna_fit.tex <==
\section{This Probably Won't Fit in the Paper (or is just weak)}

\subsubsection{Question type.}
Microsoft's internal algorithms usually output one of the 7 possible clarifying questions in response to user query \cite{zamani2020mimics}.
We investigate the performance of our model w.r.t. the clarifying question type.
The results in Figure \ref{fig:qtype} suggest that there are differences between them.
\maybe{I would maybe replace this with number of retrieved results experiment. When you look at the questions in MIMICS original paper (table 4), you can't really see much of a difference between them.}
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figs/question_type.png}
    \caption{Performance by question type.}
    \label{fig:qtype}
\end{figure}

\subsubsection{Clarification pane selection.}
\begin{table}[]
\centering
\caption{Performance on clarification pane re-ranking task on MIMICS-ClickExplore. $\dagger$ indicates statistical significance with $p<0.01$. \maybe{Random is a bad name}.}
\begin{tabular}{l@{\quad}l@{\quad}l@{\quad}l@{\quad}l@{\quad}}
\toprule
               & nDCG@1 & nDCG@2 & nDCG@3 & nDCG@5 \\
\midrule
\textit{Worst question} & 0.0    & 0.486  & 0.544  & 0.586   \\
\textit{Random} & 0.437 & 0.728  & 0.759 & 0.771 \\
ELBERT-panes   & $0.448^{\dagger}$  &  0.728  & $0.761^{\dagger}$  &  0.770 \\
ELBERT-titles  & $0.496^{\dagger}$  & $0.755^{\dagger}$  &  $0.785^{\dagger}$  & $0.794^{\dagger}$  \\
\bottomrule \\
\end{tabular}
\label{tbl:qs}
\end{table}

In this subsection, we evaluate our ELBERT model trained for predicting the engagement levels on clarification pane selection task. 
MIMICS-ClickExplore dataset contains 64k unique queries, each with multiple clarification panes, yielding a total of $168,921$ query-clarification pairs.
Each pair is associated with corresponding engagement levels, which are generated by distinct groups of users (similar to A/B testing).
Therefore, the engagement levels can be directly used as implicit feedback on the quality of clarification.
    
For each query, we rank their corresponding panes by their engagement level in descending order and consider that as true ranking, similar to \cite{zamani2020analyzing}.
As our predicted ranking, the model predicts the engagement level for each clarification pane of a given query and we rank the panes by predicted values, again in descending order.
The produced ranking is then compared to the true ranking in the dataset by nDCG@K. 
Results in Table \ref{tbl:qs} show that our model outperforms enlisted baselines, namely \textit{Worst question} and \textit{Random}.
However, relatively small improvements over baselines suggest that utilising a model trained for ELP on clarification pane selection task might not be ideal.
Zamani et. al \cite{zamani2020analyzing} report better results on the task when model is trained directly for question re-ranking, in a pair-wise setting, on manually labelled data. \maybe{Expand?}


\subsubsection{Transformer attention analysis.}
\label{attention}
%\moh{this is indeed interesting. but I wonder how we can make it smaller. maybe working on the visual side, like fading away all low-attention terms and showing only the high attention ones. also e.g., to calculate what percentage of high attention goes to which element (e.g., title, snippet, etc...) these could be used to improve presentation. any other ideas?}

%\fab{This is the most interesting part of the paper, in my view. We should find a better way to show the attention analysis, though, as the paper will be printed in b/w and the colour will not show. Maybe some other way to visualise the scale of values...}
% Remove irrelevant (or less relevant)

% It might be interesting to see where Transformer is focusing it's attention.
% Is it all around the SERPs (all 10 results)?
% Or one-two SERPs are enough?
As described in \ref{models}, we feed the model with the query, clarifying question, candidate answers, and SERP elements.
To inspect the importance of each of the input components, we perform quantitative study of ALBERT's attention mechanism on the input sequence.
Higher attention weights correspond to higher importance for making the final prediction.
We average the attention weights of all tokens of a specific component for the last 3 layers of ALBERT encoder, as they have been shown to capture most of the semantic meaning \cite{jawahar2019does}.

Figure \ref{fig:attentions} shows attention of the classification $[CLS]$ token, query tokens, clarifying question tokens, and candidate answers, over the whole input sequence, including the $10$ retrieved responses (SERPs).
The attention weights are averaged over $50$ samples in the development set.
We notice that SERP elements play an important role for each of the input components, as attention weight distribution is relatively evenly distributed among them.
Furthermore, query tokens, question tokens, and answer tokens, attend a lot to themselves.
\todo{This might be weak. We might opt to include another experiment. E.g., the first one on the next page, when it's finished.}


\begin{figure}
    \centering
    \includegraphics[scale=0.35]{figs/Screenshot 2020-10-07 at 16.45.51.png}
    \caption{Attentions of input elements over queries, clarification panes and SERP elements.}
    \label{fig:attentions}
\end{figure}

\subsection{Performance by Number of Responses}
In this subsection, we analyse the performance of our model with regard to the number of retrieved results given.
User behaviour is mainly biased by the results they see, thus it might not make sense to elicit a clarification pane if user's desired document is in user's field of vision, i.e., on top of the search results page.
We'd have something like Figure \ref{fig:tmpara}.

\begin{figure}
    \centering
    \includegraphics{figs/Screenshot 2020-10-07 at 23.44.23.png}
    \caption{Performance by number of SERP elements, as measured by $R^2$. \todo{Not real data.}}
    \label{fig:tmpara}
\end{figure}


\subsection{Error analysis}
In this subsection, we analyse the cases where our models were most wrong.
We can check if it's easier for models to predict high-engagement levels or lower ones.

\subsection{Feature analysis}
\textbf{Correlation with engagement levels.}
Heatmap figure of some simple features \ref{fig:heatmap1}.
Some features show weak to moderate correlation with the engagement levels.
Features extracted are supposed to represent the level of diversity of the returned results.
Intuitively, the higher diversity among retrieved documents, the higher necessity for the clarification, thus leading to higher engagement levels.
Features are: number of unique nouns divided by the total number of nouns in all of the snippets for a query; number of unique topics as extracted by LDA divided by the total number of topics in all of the snippets for a query.
These show weak negative correlation with engagement levels.

\maybe{I'm not sure such a heatmap is needed. That is apart from the fact that maybe the correlation are too weak anyways, as just the lengths of the documents retrieved almost correlates the best with engagement levels. These correlations are with features extracted from snippets (left) and titles (right).}

There's also boxplot possibility: Figure \ref{fig:boxplot}. There is statistically significant difference in means of groups, e.g., $(0.4,0.5]$ and $(0.7,0.8]$, where $(a,b]$ means that the ratio of unique, stemmed nouns and total stemmed nouns in SERPs falls between $a and b$.


\begin{figure}
    \centering
    \includegraphics[scale=0.35]{figs/snip_titl_placeholder.png}
    \caption{Correlation of features extracted from SERP snippets and associated the engagement levels.}
    \label{fig:heatmap1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.35]{figs/titles_snippets_boxplot_NN.png}
    \caption{Ratio of unique nouns and total nouns against the engagement levels. The higher the diversity (lower x-axis), higher the EL.}
    \label{fig:boxplot}
\end{figure}

\textbf{Answer coverage.}
We check for coverage of options (answers) in clarification panes in SERPs.
Engagement levels are higher with clarification panes whose all of the options are actually present in the first 10 results.
Panes whose options are not in the first $10$ results get engaged with less.
We group the dataset samples in three groups, where:
\begin{enumerate}
    \item \textit{all} of the answers are contained in the retrieved results;
    \item \textit{some}, but not all, of the answers are covered in the SERPs;
    \item \textit{none} of the answers are present in SERPs.
\end{enumerate}

\begin{table}[]
\centering
\begin{tabular}{llll}
\toprule
Groups    & $\mu_1$  & $\mu_2$  & $p$-value \\
\midrule
\textit{all}-\textit{some}  & 5.71 & 5.43 & 7.4e-6  \\
\textit{all}-\textit{none}  & 5.71 & 5.36 & 3.4e-9  \\
\textit{some}-\textit{none} & 5.43 & 5.36 & 0.001  \\
\bottomrule \\
\end{tabular}
\caption{Means and the p-values of a paired t-test of answer coverage groups.}
\label{tbl:coverage}
\end{table}

We compare the groups of the engagement levels using a paired t-test.
All of the group pairs compared can be found in Table \ref{tbl:coverage}.
The means of the first group, where all of the answers are contained in SERPs, are significantly higher than in other groups, $p < 0.001$.
This indicates the quality of the clarification pane itself, as users tend to interact more with panes that are present on the first page of results.


%{\tiny \mybox{color9}{\strut{[CLS]}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color1}{\strut{nh}} \mybox{color9}{\strut{[SEP]}} \mybox{color0}{\strut{select}} \mybox{color0}{\strut{one}} \mybox{color0}{\strut{to}} \mybox{color0}{\strut{re}} \mybox{color0}{\strut{fine}} \mybox{color0}{\strut{your}} \mybox{color0}{\strut{search}} \mybox{color9}{\strut{[SEP]}} \mybox{color0}{\strut{zip}} \mybox{color0}{\strut{code}} \mybox{color0}{\strut{things}} \mybox{color0}{\strut{to}} \mybox{color0}{\strut{do}} \mybox{color0}{\strut{hotel}} \mybox{color0}{\strut{homes}} \mybox{color0}{\strut{for}} \mybox{color0}{\strut{sale}} \mybox{color9}{\strut{[SEP]}} \mybox{color1}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color1}{\strut{nh}} \mybox{color0}{\strut{}} \mybox{color2}{\strut{.}} \mybox{color0}{\strut{com}} \mybox{color0}{\strut{}} \mybox{color1}{\strut{**}} \mybox{color0}{\strut{please}} \mybox{color0}{\strut{read}} \mybox{color0}{\strut{our}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{co}} \mybox{color0}{\strut{vid}} \mybox{color0}{\strut{-}} \mybox{color0}{\strut{19}} \mybox{color0}{\strut{page}} \mybox{color0}{\strut{for}} \mybox{color0}{\strut{updates}} \mybox{color0}{\strut{on}} \mybox{color0}{\strut{what}} \mybox{color0}{\strut{is}} \mybox{color0}{\strut{currently}} \mybox{color0}{\strut{open}} \mybox{color0}{\strut{in}} \mybox{color0}{\strut{the}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{area}} \mybox{color4}{\strut{.}} \mybox{color4}{\strut{.}} \mybox{color0}{\strut{our}} \mybox{color0}{\strut{online}} \mybox{color0}{\strut{area}} \mybox{color0}{\strut{guide}} \mybox{color0}{\strut{is}} \mybox{color0}{\strut{full}} \mybox{color0}{\strut{of}} \mybox{color0}{\strut{valuable}} \mybox{color0}{\strut{information}} \mybox{color0}{\strut{on}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{nh}} \mybox{color1}{\strut{hotels}} \mybox{color0}{\strut{&}} \mybox{color0}{\strut{lodging}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{restaurants}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{shopping}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{skiing}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{golf}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{area}} \mybox{color0}{\strut{attractions}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{outdoor}} \mybox{color0}{\strut{recreation}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{local}} \mybox{color0}{\strut{businesses}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{photos}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{videos}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{maps}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{news}} \mybox{color0}{\strut{&}} \mybox{color0}{\strut{events}} \mybox{color1}{\strut{and}} \mybox{color0}{\strut{much}} \mybox{color0}{\strut{more}} \mybox{color5}{\strut{.}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{motel}} \mybox{color0}{\strut{s}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{campground}} \mybox{color0}{\strut{s}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{family}} \mybox{color0}{\strut{hotels}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{business}} \mybox{color0}{\strut{hotels}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{resort}} \mybox{color0}{\strut{s}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{spa}} \mybox{color0}{\strut{resort}} \mybox{color0}{\strut{s}} \mybox{color0}{\strut{romantic}} \mybox{color0}{\strut{hotels}} \mybox{color0}{\strut{in}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{luxury}} \mybox{color0}{\strut{hotels}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{ski}} \mybox{color0}{\strut{-}} \mybox{color0}{\strut{in}} \mybox{color2}{\strut{}} \mybox{color0}{\strut{/}} \mybox{color0}{\strut{ski}} \mybox{color0}{\strut{-}} \mybox{color0}{\strut{out}} \mybox{color0}{\strut{hotels}} \mybox{color0}{\strut{5}} \mybox{color0}{\strut{-}} \mybox{color0}{\strut{stars}} \mybox{color0}{\strut{hotels}} \mybox{color0}{\strut{in}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{4}} \mybox{color0}{\strut{-}} \mybox{color0}{\strut{stars}} \mybox{color0}{\strut{hotels}} \mybox{color0}{\strut{in}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{3}} \mybox{color0}{\strut{-}} \mybox{color0}{\strut{stars}} \mybox{color0}{\strut{hotels}} \mybox{color0}{\strut{in}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{choice}} \mybox{color0}{\strut{}} \mybox{color1}{\strut{.}} \mybox{color0}{\strut{.}} \mybox{color3}{\strut{.}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{part}} \mybox{color0}{\strut{of}} \mybox{color0}{\strut{new}} \mybox{color0}{\strut{hampshire}} \mybox{color0}{\strut{'}} \mybox{color0}{\strut{s}} \mybox{color0}{\strut{scenic}} \mybox{color0}{\strut{mount}} \mybox{color0}{\strut{washington}} \mybox{color0}{\strut{valley}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{has}} \mybox{color0}{\strut{been}} \mybox{color0}{\strut{dubbed}} \mybox{color0}{\strut{the}} \mybox{color0}{\strut{offspring}} \mybox{color0}{\strut{of}} \mybox{color0}{\strut{a}} \mybox{color0}{\strut{quint}} \mybox{color0}{\strut{essential}} \mybox{color0}{\strut{new}} \mybox{color0}{\strut{england}} \mybox{color0}{\strut{village}} \mybox{color0}{\strut{and}} \mybox{color0}{\strut{a}} \mybox{color0}{\strut{gap}} \mybox{color0}{\strut{outlet}} \mybox{color3}{\strut{.}} \mybox{color0}{\strut{historic}} \mybox{color0}{\strut{buildings}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{qua}} \mybox{color0}{\strut{int}} \mybox{color0}{\strut{antique}} \mybox{color0}{\strut{shops}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{bookstore}} \mybox{color0}{\strut{s}} \mybox{color0}{\strut{and}} \mybox{color0}{\strut{baker}} \mybox{color0}{\strut{ies}} \mybox{color0}{\strut{co}} \mybox{color0}{\strut{ex}} \mybox{color0}{\strut{ist}} \mybox{color0}{\strut{peacefully}} \mybox{color0}{\strut{with}} \mybox{color0}{\strut{big}} \mybox{color0}{\strut{name}} \mybox{color0}{\strut{outlet}} \mybox{color0}{\strut{stores}} \mybox{color0}{\strut{like}} \mybox{color0}{\strut{j}} \mybox{color0}{\strut{.}} \mybox{color0}{\strut{jill}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{nike}} \mybox{color0}{\strut{and}} \mybox{color0}{\strut{dan}} \mybox{color0}{\strut{sk}} \mybox{color7}{\strut{.}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{is}} \mybox{color0}{\strut{a}} \mybox{color0}{\strut{census}} \mybox{color0}{\strut{-}} \mybox{color0}{\strut{designated}} \mybox{color0}{\strut{place}} \mybox{color0}{\strut{}} \mybox{color0}{\strut{(}} \mybox{color0}{\strut{cdp}} \mybox{color0}{\strut{)}} \mybox{color0}{\strut{and}} \mybox{color0}{\strut{village}} \mybox{color0}{\strut{in}} \mybox{color0}{\strut{eastern}} \mybox{color0}{\strut{carroll}} \mybox{color0}{\strut{county}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{new}} \mybox{color1}{\strut{hampshire}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{united}} \mybox{color0}{\strut{states}} \mybox{color2}{\strut{.}} \mybox{color0}{\strut{the}} \mybox{color0}{\strut{population}} \mybox{color0}{\strut{was}} \mybox{color0}{\strut{2}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{349}} \mybox{color0}{\strut{at}} \mybox{color0}{\strut{the}} \mybox{color0}{\strut{2010}} \mybox{color0}{\strut{census}} \mybox{color7}{\strut{.}} \mybox{color0}{\strut{a}} \mybox{color0}{\strut{year}} \mybox{color0}{\strut{-}} \mybox{color0}{\strut{round}} \mybox{color0}{\strut{resort}} \mybox{color0}{\strut{area}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{is}} \mybox{color0}{\strut{the}} \mybox{color0}{\strut{largest}} \mybox{color0}{\strut{village}} \mybox{color0}{\strut{within}} \mybox{color0}{\strut{the}} \mybox{color0}{\strut{town}} \mybox{color0}{\strut{of}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{which}} \mybox{color0}{\strut{is}} \mybox{color0}{\strut{bounded}} \mybox{color0}{\strut{on}} \mybox{color0}{\strut{the}} \mybox{color0}{\strut{east}} \mybox{color0}{\strut{by}} \mybox{color0}{\strut{the}} \mybox{color0}{\strut{maine}} \mybox{color0}{\strut{state}} \mybox{color0}{\strut{line}} \mybox{color9}{\strut{.}} \mybox{color0}{\strut{the}} \mybox{color0}{\strut{white}} \mybox{color0}{\strut{mountain}} \mybox{color0}{\strut{national}} \mybox{color0}{\strut{forest}} \mybox{color0}{\strut{is}} \mybox{color0}{\strut{to}} \mybox{color0}{\strut{the}} \mybox{color0}{\strut{west}} \mybox{color0}{\strut{and}} \mybox{color0}{\strut{north}} \mybox{color7}{\strut{.}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{,}} \mybox{color2}{\strut{nh}} \mybox{color1}{\strut{}} \mybox{color0}{\strut{<unk>}} \mybox{color0}{\strut{attractions}} \mybox{color0}{\strut{cran}} \mybox{color0}{\strut{more}} \mybox{color0}{\strut{mountain}} \mybox{color0}{\strut{resort}} \mybox{color5}{\strut{.}} \mybox{color0}{\strut{this}} \mybox{color0}{\strut{mountain}} \mybox{color0}{\strut{is}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{in}} \mybox{color0}{\strut{a}} \mybox{color0}{\strut{word}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{fun}} \mybox{color6}{\strut{.}} \mybox{color0}{\strut{known}} \mybox{color0}{\strut{for}} \mybox{color0}{\strut{expert}} \mybox{color0}{\strut{snow}} \mybox{color0}{\strut{making}} \mybox{color0}{\strut{and}} \mybox{color0}{\strut{a}} \mybox{color0}{\strut{range}} \mybox{color0}{\strut{of}} \mybox{color0}{\strut{trails}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{cran}} \mybox{color0}{\strut{more}} \mybox{color0}{\strut{also}} \mybox{color0}{\strut{has}} \mybox{color0}{\strut{thrill}} \mybox{color0}{\strut{ing}} \mybox{color0}{\strut{off}} \mybox{color0}{\strut{-}} \mybox{color0}{\strut{s}} \mybox{color0}{\strut{lope}} \mybox{color0}{\strut{activities}} \mybox{color0}{\strut{such}} \mybox{color0}{\strut{as}} \mybox{color0}{\strut{mountain}} \mybox{color0}{\strut{coaster}} \mybox{color0}{\strut{rides}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{giant}} \mybox{color0}{\strut{swing}} \mybox{color0}{\strut{rides}} \mybox{color1}{\strut{,}} \mybox{color0}{\strut{and}} \mybox{color0}{\strut{the}} \mybox{color0}{\strut{soaring}} \mybox{color0}{\strut{eagle}} \mybox{color0}{\strut{zip}} \mybox{color0}{\strut{line}} \mybox{color7}{\strut{}} \mybox{color0}{\strut{<unk>}} \mybox{color0}{\strut{all}} \mybox{color0}{\strut{just}} \mybox{color0}{\strut{a}} \mybox{color0}{\strut{few}} \mybox{color0}{\strut{miles}} \mybox{color0}{\strut{from}} \mybox{color0}{\strut{downtown}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color9}{\strut{.}} \mybox{color2}{\strut{book}} \mybox{color0}{\strut{your}} \mybox{color2}{\strut{hotel}} \mybox{color0}{\strut{in}} \mybox{color0}{\strut{north}} \mybox{color1}{\strut{conway}} \mybox{color0}{\strut{and}} \mybox{color0}{\strut{pay}} \mybox{color0}{\strut{later}} \mybox{color0}{\strut{with}} \mybox{color0}{\strut{ex}} \mybox{color1}{\strut{pedia}} \mybox{color9}{\strut{.}} \mybox{color1}{\strut{enjoy}} \mybox{color0}{\strut{free}} \mybox{color1}{\strut{cancellation}} \mybox{color0}{\strut{on}} \mybox{color0}{\strut{most}} \mybox{color2}{\strut{hotels}} \mybox{color9}{\strut{.}} \mybox{color0}{\strut{save}} \mybox{color0}{\strut{big}} \mybox{color0}{\strut{on}} \mybox{color0}{\strut{a}} \mybox{color0}{\strut{wide}} \mybox{color0}{\strut{range}} \mybox{color0}{\strut{of}} \mybox{color1}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color2}{\strut{hotels}} \mybox{color3}{\strut{!}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color0}{\strut{is}} \mybox{color0}{\strut{known}} \mybox{color0}{\strut{for}} \mybox{color0}{\strut{its}} \mybox{color1}{\strut{mountain}} \mybox{color0}{\strut{views}} \mybox{color0}{\strut{and}} \mybox{color0}{\strut{forests}} \mybox{color9}{\strut{.}} \mybox{color1}{\strut{book}} \mybox{color1}{\strut{hotels}} \mybox{color0}{\strut{and}} \mybox{color0}{\strut{other}} \mybox{color0}{\strut{accommodation}} \mybox{color0}{\strut{s}} \mybox{color0}{\strut{near}} \mybox{color1}{\strut{scho}} \mybox{color0}{\strut{ul}} \mybox{color0}{\strut{er}} \mybox{color0}{\strut{park}} \mybox{color0}{\strut{,}} \mybox{color0}{\strut{echo}} \mybox{color0}{\strut{lake}} \mybox{color0}{\strut{state}} \mybox{color0}{\strut{park}} \mybox{color2}{\strut{,}} \mybox{color0}{\strut{and}} \mybox{color0}{\strut{merri}} \mybox{color0}{\strut{man}} \mybox{color0}{\strut{state}} \mybox{color0}{\strut{forest}} \mybox{color0}{\strut{today}} \mybox{color9}{\strut{.}} \mybox{color0}{\strut{other}} \mybox{color0}{\strut{sight}} \mybox{color0}{\strut{s}} \mybox{color0}{\strut{in}} \mybox{color0}{\strut{the}} \mybox{color0}{\strut{area}} \mybox{color0}{\strut{include}} \mybox{color0}{\strut{cran}} \mybox{color0}{\strut{more}} \mybox{color0}{\strut{mountain}} \mybox{color0}{\strut{resort}} \mybox{color9}{\strut{.}} \mybox{color0}{\strut{best}} \mybox{color2}{\strut{campground}} \mybox{color0}{\strut{s}} \mybox{color0}{\strut{in}} \mybox{color0}{\strut{north}} \mybox{color0}{\strut{conway}} \mybox{color2}{\strut{,}} \mybox{color1}{\strut{conway}} \mybox{color1}{\strut{,}} \mybox{color3}{\strut{nh}} \mybox{color5}{\strut{}} \mybox{color1}{\strut{-}} \mybox{color0}{\strut{yo}} \mybox{color0}{\strut{gi}} \mybox{color0}{\strut{bear}} \mybox{color1}{\strut{'}} \mybox{color0}{\strut{s}} \mybox{color0}{\strut{jelly}} \mybox{color0}{\strut{stone}} \mybox{color0}{\strut{park}} \mybox{color1}{\strut{-}} \mybox{color0}{\strut{camp}} \mybox{color0}{\strut{resort}} \mybox{color0}{\strut{glen}} \mybox{color0}{\strut{ellis}} \mybox{color1}{\strut{,}} \mybox{color0}{\strut{woodland}} \mybox{color0}{\strut{acres}} \mybox{color0}{\strut{campground}} \mybox{color2}{\strut{,}} \mybox{color0}{\strut{covered}} \mybox{color0}{\strut{bridge}} \mybox{color1}{\strut{campground}} \mybox{color3}{\strut{,}} \mybox{color0}{\strut{the}} \mybox{color0}{\strut{beach}} \mybox{color0}{\strut{family}} \mybox{color0}{\strut{campground}} \mybox{color4}{\strut{,}} \mybox{color0}{\strut{}} \mybox{color0}{\strut{s}} \mybox{color0}{\strut{aco}} \mybox{color0}{\strut{river}} \mybox{color1}{\strut{camping}} \mybox{color0}{\strut{area}} \mybox{color8}{\strut{,}} \mybox{color9}{\strut{[SEP]}}}



% \begin{table}[]
% \centering
% \begin{tabular}{lllllll}
% \toprule
%                       & \multicolumn{3}{l}{Full MIMICS-Click}               & \multicolumn{3}{l}{With EL > 0} \\
%                       \midrule
% Model                 & MAE             & MSE             & $R^2$           & MAE      & MSE      & $R^2$     \\
% \midrule
% Mean                  & 0.1531          & 0.0546          & 0.0             & 0.2410  & 0.0780   &  0.0  \\
% Median                & \textbf{0.0921} & 0.0531          & 0.0             & 0.2396 &  0.0793  &  0.0    \\
% Normal                & 0.1896          & 0.0823          & 0.0             & 0.4275   & 0.2596   &  0.0 \\
% \midrule
% Linear Regression     & 0.1463          & 0.0530          & 0.0359          & 0.2364   &  0.0783  &  0.0083      \\
% LinearSVR             & 0.1462          & 0.0522          & 0.0490           & 0.2318  &  0.0736  & 0.0676  \\
% RandomForestRegressor & tbd             & tbd             & tbd             &  0.2301  &  0.0729  &  0.0775   \\
% ELBERT                & 0.1397 & \textbf{0.0518} & \textbf{0.0513}          & \textbf{0.2255}   &  \textbf{0.0706}  &  \textbf{0.09445} \\
% \bottomrule \\
% \end{tabular}
% \caption{Performance on the full MIMICS-Click dataset (400k+ samples) and a subset where engagement levels are higher than zero (71k samples). Evaluation is done in a 5-fold cross-validation setting with $+$ marking statistical significance with $p < 0.01$. \todo{The plan is to also add another popular neural baseline, CNN.}}
% \label{tbl:results}
% \end{table}

% OLD
%\subsection{Our approach}
%\label{approach}

% We point that the user engagement levels can be estimated by either:
% \begin{itemize}
%     \item Looking at the query only;
%     \item Utilising the clarification pane information in addition to the query;
%     \item Exploring SERPs for even more data.  
% \end{itemize}

%We argue that the engagement level prediction task has two main points of view.
%First, when utilising the clarification pane for a more accurate prediction, we are implicitly trying to estimate the \textit{quality} of the pane with regard to the query and, potentially, the retrieved results.
%In this setting, a clarification question has already been asked and we are interested into how engaging it actually is.
%The assumption is that, the higher the engagement level, the better the question and the provided answers are. 
%\maybe{I guess that's similar to using clicks for estimating document relevance in retrieval, so we might wanna cite something.}

%On the other hand, considering the initial query with the retrieved results only, i.e., without the information about the clarification pane, focuses more on the \textit{necessity} of asking a clarification question.
%Determining whether to ask a question is very much applicable to the real-world scenario in modern search engines, and even more in conversational search and search on mobile devices, i.e., interfaces with limited bandwidth.
%We can draw an analogy between the distinction of query performance prediction methods, i.e., pre-retrieval and post-retrieval methods \cite{carmel2010estimating}, and this context as well.
%In the pre-retrieval setting, we must infer the engagement level based on the query only, while in the post-retrieval setting we can utilise the retrieved results as well.
%We perform experiments in the pre-, as well as the post-retrieval setting.

% Although the two points of view can lead to very different directions in future research on the topic, we provide strong baselines with, and without clarification pane information.
% \maybe{Recently, Zamani et al. \cite{zamani2020analyzing} study query-pane-answer combinations for clarifying question selection.
% They provide interesting findings, relevant to this study as well.
% For example, ambiguous and faceted queries with multiple aspects lead to higher interactions with the clarification pane.
% This further motivates us to model the diversity of the retrieved results, with necessity of clarification in mind.}

% \moh{I think the proposed approach is not explained well. this section is mainly discussing what others have and the motivations behind our model. I would say they should mostly be expressed in Intro where we want to sell the paper and also provide motavation for it. here I would only mention how the model works and with some straight description of our choices. I suggest you check my CHIIR'20 or SIGIR'19 method section to see how you could describe the model. it doesn't matter if it is only using Albert, you can still formalize it in a mathematical way so that people can follow it more clearly.}
